The Algebras for Automatic Relations

We introduce "synchronous algebras", an algebraic structure tailored to recognize automatic relations (aka. synchronous relations, or regular relations). They are the equivalent of monoids for regular languages, however they conceptually differ in two points: first, they are typed and second, they are equipped with a dependency relation expressing constraints between elements of different types. The interest of the proposed definition is that it allows to lift, in an effective way, pseudovarieties of regular languages to that of synchronous relations, and we show how algebraic characterizations of pseudovarieties of regular languages can be lifted to the pseudovarieties of synchronous relations that they induce. A typical example of such a pseudovariety is the class of "group relations", defined as the relations recognized by finite-state synchronous permutation automata. In order to prove this result, we adapt two pillars of algebraic language to synchronous algebras: (a) any relation admits a syntactic synchronous algebra recognizing it, and moreover, the relation is synchronous if, and only if, its syntactic algebra is finite and (b) classes of synchronous relations with desirable closure properties (i.e. pseudovarieties) correspond to pseudovarieties of synchronous algebras.

==> sec/apdx-henckell.tex <==
\section{Henckell Pseudovarieties}
\label{apdx:henckell}

% \todo{clean \& complete}

To describe the additional hypothesis that we need to prove the implication $(3) \Rightarrow (1)$ 
of \Cref{thm:lifting-semigroup}, we first need to introduce "pointlike sets", a crucial tool
from semigroup theory. We refer to "eg" \cite{almeida_pointlike_2008} for formal definitions.
% We provide formal
% definitions in \todo{the appendix}, but in this section
% we will rather focus on the property they satisfy to provide an intuitive understanding of our 
% results.

Given a finite semigroup $S$ and a "pseudovariety of semigroups" $\B{V}$, a natural question is to ask
whether $S$ belongs to $\B{V}$. The \AP""$\B{V}$-pointlike sets"",
can be understood as a quantitative version of this: they form a collection of (non-empty) subsets $X \subseteq S$ whose elements cannot be ``distinguished'' using semigroups from $\B{V}$. In particular, all singletons are 
"pointlikes", and $S \in \B{V}$ "iff" its $\B{V}$-pointlikes only consists of these singletons.
In general, "pointlikes" form a subsemigroup of the powerset semigroup $\pset(S)$ of $S$, and
are downward-closed: if $X$ is a non-empty subset of $Y$ and $Y$ is "pointlike", then so is $X$.
The collection of "$\B{V}$-pointlike sets" of $S$ is denoted by \AP$\intro*\Pl(S)$.

Note that if $\Pl$ is computable, then $\B{V}$-membership is decidable---to test if
$S \in \B{V}$ it suffices to test if $\Pl(S)$ is the semigroup of singletons of $S$---but the latter problem is remarkably more complex. Conceptually, there are "pseudovarieties@@sg" 
for which membership is beyond trivial---"eg" aperiodic semigroups or groups---but for which the computability of the "pointlike sets" are considered to be seminal results of semigroup theory---"eg" Henckell theorem on the "aperiodic" "pointlikes" \cite[Fact 3.7, p.~96 \& Fact 5.31, p.~122]{henckell_pointlike_1988}, or Ash type II theorem on the group "pointlikes" \cite[Theorem 2.1, p.~129]{ash_inevitable_1991}, see \cite[Theorem 1.1, p.~3]{henckell_ashs_1991} for a clear reformulation in terms of "pointlike sets". Moreover, there exists pseudovarieties
with decidable membership but whose pointlikes are not computable \cite[Corollary 1.6, p.~478]{rhode_pointlike_2011}.

Almeida then noticed the relationship between this established tool in semigroup theory and the separation problems in language theory.
\begin{proposition}[{\cite[Lemma 3.1, p.~3]{almeida_algorithmic_1999}}]
	\label{prop:separation-pointlikes}
	Given two languages $L_1, L_2 \subseteq \Sigma^+$ recognized by a single
	morphism $\phi\colon \Sigma^+ \to S$, the following are equivalent:
	\begin{itemize}
		\item $L_1$ and $L_2$ are $\+V$-separable,
		\item no "$\B{V}$-pointlike set" $X$ of $S$ intersects both $\phi[L_1]$
			and $\phi[L_2]$.
	\end{itemize} 
\end{proposition}

\begin{corollary}[of \Cref{fact:separability} and \Cref{prop:separation-pointlikes}]
	\label{coro:pointlike-consolidation}
	A "relation" $\+R$ is a "$\+V$-relation" "iff" there is no
	$X \in \Pl(\consolSyntSAP{\+R})$ that intersects both
	$\sgpSyntSAMP{\+R}[\+R]$ and $\sgpSyntSAMP{\+R}[\negrel\+R]$.
\end{corollary}

One notable feature of Henckell theorem relies in the relative simplicity of the characterization
of the "aperiodic" "pointlike sets". Recall that \AP""aperiodic semigroups""
are defined by the "profinite equality" $x^{\idem} = x^{\idem +1}$---they exactly correspond
by the Schützenberger-McNaughton-Papert theorem to the star-free languages \cite[Main Property, p.~190]{schutzenberger_finite_1965}, or
equivalently to the first-order definable languages \cite{mcnaughton_counter-free_1971}---see \cite[Theorem 2.6, p.~40]{bojanczyk_languages_2020} for a modern presentation. Then the "aperiodic" "pointlike sets" of $S$ exactly corresponds to the smallest downward-closed
subsemigroup $\+P$ of $\pset(S)$ containing all singletons, and such that
if $X \in \+P$, then $X^{\idem}\cup X^{\idem+1} \in \+P$.\footnote{Beware: $X^{\idem}$
refers to the "idempotent power" of $X$, seen as an element of the powerset semigroup.~In particular, it is in general strictly bigger than $\{x^{\idem} \mid x \in X\}$.} Notice the
obvious relationship between the "profinite equality" $x^{\idem} = x^{\idem+1}$ and the operator
$X \mapsto X^{\idem} \cup X^{\idem+1}$. This begs the question of whether this procedure can be 
generalized to any "pseudovariety@@sgp".

\begin{definition}
	Given a "pseudovariety of semigroups" $\B{V}$ "defined@@profeq" by a set $\+E$ of "profinite 
	equalities", define the \AP""$\+E$-closure"" of a finite semigroup $S$, denoted by
	\AP$\intro*\Cl{\+E}(S)$, as the smallest downward-closed subsemigroup $\+P$
	of $\pset(S)$ containing
	all singletons and such that for each $(u \profeq v) \in \+E$ over variables $X$,
	for each morphism $\phi\colon X^+ \to \pset(S)$, if $\phi(x) \in \+P$ for all $x \in X$,
	then $\profSg{\phi}(u)\cup\profSg{\phi}(v) \in \+P$.
\end{definition}

Then Henckell theorem can be simply restated as $\Cl[\B{A}]{\+E} = \Pl[\B{A}]$ where $\B{A}$ 
denotes the "pseudovariety@@sgp" of "aperiodic semigroups" and
$\+E = \{x^{\omega} = x^{\omega+1}\}$. In general, the equality is false, but one inclusion always hold.

\begin{fact}[Folklore]
	\label{fact:closure-included-pointlikes}
	For every semigroup $S$, $\Cl{\+E}(S) \subseteq \Pl(S)$.
\end{fact}
% \todo{proof in appendix}

We say that a "pseudovariety@@sgp" is \AP""Henckell for $\+E$"" if $\Cl{\+E} = \Pl$.
Notice that if $\+E, \+F$ are two sets of "profinite equalities" defining $\B{V}$,
if $\+E \subseteq \+F$, then $\Cl{\+E}(S) \subseteq \Cl{\+F}(S)$. Under these assumptions,
if $\B{V}$ is "Henckell for $\+E$", then it is "Henckell for $\+F$",
by \Cref{fact:closure-included-pointlikes}. We say that a "pseudovariety@@sgp" $\B{V}$
is ""Henckell""\footnote{While the question of understanding which "pseudovarieties@@sgp" satisfy 
$\Cl{\+E} = \Pl$ is regularly studied in the semigroup literature---mainly as a way to characterize 
the "pointlikes", see "eg" \cite[Theorem 3.2, p.~7]{gool_pointlike_2019} for pseudovarieties of 
semigroups determined by groups, or \cite[Theorem 3.1, p.~489]{almeida_pointlike_2008} showing that 
$\+R$-trivial semigroups are "Henckell" but $\+J$-trivial semigroups, corresponding to 
piecewise-testable languages, are not "Henckell" \cite[\S 6.1, p.~495]{almeida_pointlike_2008}---and is a hard problem,
we do not know of any  standard terminology to describe these classes.} if there exists $\+E$ such 
that it is "Henckell for $\+E$", or, equivalently, if it is "Henckell for $\EqVar{\B{V}}$".

\begin{lemma}
	\label{lemma:induced-profdep-implies-Vrelation-Henckell}
	Let $\B{V}$ be a "pseudovariety@@sgp" which is "Henckell for $\+E$".
	Then, using the notations of \Cref{thm:lifting-semigroup},
	if the "syntactic positive synchronous algebra" of $\+R$ "satisfies@@profdep"
	all "profinite dependencies" of $\inducedProfdep{\+E}$, then $\+R$ is a "$\+V$-relation". 
\end{lemma}

\begin{proof}
	The idea is to use \Cref{coro:pointlike-consolidation}:
	deciding whether $\+R$ is a "$\+V$-relation" can be done
	by looking at the "$\B{V}$-pointlike sets" of the "consolidation"
	of the "syntactic positive synchronous algebra" of $\+R$.

	Assume that $\SyntSAP{\+R}$ satisfies all
	"profinite dependencies" of $\inducedProfdep{\+E}$.
	We claim that no set from $\Cl{\+E}(\consolSyntSAP{\+R})$ 
	can intersect both $\sgpSyntSAMP{\+R}[\+R]$ and $\sgpSyntSAMP{\+R}[\negrel\+R]$.
	Formally, we will show by induction on $X \in \Cl{\+E}(\consolSyntSAP{\+R})$ that:
	\begin{equation}
		\text{All non-zero elements of $X$ are pairwise dependent in $\SyntSAP{\+R}$.}
		\tag{\adforn{3}}
		\label{eq:hyp-ind-pointlike}
	\end{equation}
	\begin{itemize}
		\item The property holds for the subsemigroup of singletons.
		\item The property is stable under product: if both $X$ and $Y$ satisfy the property,
			then let $xy \in XY$ and $x'y' \in XY$. If one of them is zero, then we are done.
			Otherwise $x \dep x'$ and $y \dep y'$ implies $xy \dep x'y'$ since both $xy$ and $x'y'$ are well-defined.
		\item Lastly, let $(u \profeq v) \in \+E$ and $\psi\colon X^+ \to \+P(\consolSyntSAP{\+R})$
			be such that $\phi(x)$ satisfies \eqref{eq:hyp-ind-pointlike} for all $x \in X$.
			We want to show that $\profSg{\phi}(u) \cup \profSg{\phi}(v)$ satisfy
			\eqref{eq:hyp-ind-pointlike}.
			Pick two non-zero elements in $\profSg{\phi}(u) \cup \profSg{\phi}(v)$. If both
			belong to $\profSg{\phi}(u)$ (or dually to $\profSg{\phi}(v)$) then the same argument as in the point above show that they are "dependent". So "wlog", pick $s \in \profSg{\phi}(u)$ and $t \in \profSg{\phi}(v)$. By construction, there exists "morphisms@@syncP" $\psi_u\colon X^+ \to \consolSyntSAP{\+R}$ and $\psi_v\colon X^+ \to \consolSyntSAP{\+R}$ such that $\profSg{\psi_u}(u) = s$, $\profSg{\psi_v}(v) = t$
			and $\{\profSg{\psi_u}(x), \profSg{\psi_v}(x)\} \subseteq \profSg{\phi}(x)$ for all $x \in X$. By \eqref{eq:hyp-ind-pointlike} $\profSg{\psi_u}(x) \dep \profSg{\psi_v}(x)$, so by induction on well-formed words $w \in X^+$---here \emph{well-formed} means $\psi_u(w) \neq 0$ and $\psi_v(w) \neq 0$---, and by density of finite words in profinite words, it follows that
			\[\profSg{\psi_u}(u) \dep \profSg{\psi_v}(u).\]
			\todo{For this we need $\psi_v(u) \neq 0$. Why true?}
			But then, since $(u = v) \in \+E$ and since $\consolSyntSAP{\+R}$
			"satisfies@@profdep" $\inducedProfdep{\+E}$, it follows that
			\[\profSg{\psi_v}(u) \dep \profSg{\psi_v}(v).\]
			Note that $\profSg{\psi_u}(u)$ and $\profSg{\psi_v}(u)$ have the same type,
			\todo{why?} so by "local transitivity", the two "dependencies" above imply
			$\profSg{\psi_u}(u) \dep \profSg{\psi_v}(v)$, "ie" $s \dep t$.
	\end{itemize}
	Hence, it follows that all sets $X \in \Cl{\+E}(\consolSyntSAP{\+R})$ satisfy
	\Cref{eq:hyp-ind-pointlike}.

	In particular, since both
	$\sgpSyntSAMP{\+R}[\+R]$ and $\sgpSyntSAMP{\+R}[\negrel\+R]$ do not contain zero
	and are closed subsets of $\SyntSAP{\+R}$, it follows that no $X \in \Cl{\+E}(\consolSyntSAP{\+R})$ can intersect $\sgpSyntSAMP{\+R}[\+R]$ and $\sgpSyntSAMP{\+R}[\negrel\+R]$
	at the same time.
	The conclusion follows from \Cref{coro:pointlike-consolidation}
	since $\B{V}$ is "Henckell for $\+E$"
	and hence $\Cl{\+E}(\consolSyntSAP{\+R}) = \Pl(\consolSyntSAP{\+R})$.
\end{proof}

Putting together the implications
$(1) \Rightarrow (2) \Rightarrow (3)$ of \Cref{thm:lifting-semigroup} with
\Cref{lemma:induced-profdep-implies-Vrelation-Henckell}, we obtain the following result.

\begin{restatable}[The Lifting theorem for Henckell Pseudovarieties]{theorem}{liftingtheoremhenckell}
	\label{thm:lifting-theorem-henckell}
	Given a "relation" $\+R \subseteq (\Sigma^*\times\Sigma^*)\smallsetminus\{(\varepsilon, \varepsilon)\}$ and a "$+$-pseudovariety of regular languages" $\+V$
	"corresponding@@EilenbergSg" to a "pseudovariety of semigroups" $\B{V}$
	which is "Henckell for $\+E$", then the following are equivalent:
	\begin{enumerate}
		\item $\+R$ is a "$\+V$-relation",
		\item $\+R$ is "recognized@@sync" by a finite "positive synchronous algebra" $\mathbf{A}$
			"satisfying@@profdep" all "profinite dependencies" $\inducedProfdep{\+E}$ 
			"induced@@profdep" by $\+E$,
		\item the "syntactic positive synchronous algebra" of $\+R$ "satisfies@@profdep"
			all "profinite dependencies" of $\inducedProfdep{\+E}$.
	\end{enumerate} 
\end{restatable}

Lastly, observe that if $\+E$ is finite, then so is $\inducedProfdep{\+E}$.

% \subsection{Locally Trivial Languages}
% \label{apdx:sec:locally-trivial-relations}

% \AP""Locally trivial semigroups"" \AP$\intro*\LocTrivS$ can be equivalently defined by
% $\+E \defeq \{ x^{\idem} y x^{\idem} = x^{\idem} \}$, or by
% $\+F \defeq \{ x^{\idem} y z^{\idem} = x^{\idem} z^{\idem} \}$, see
% \cite[Proposition XI.4.17, p.~197]{pin_mathematical_2022}.

% Observe first that $\Cl[\LocTrivS]{\+E} \subseteq \Cl[\LocTrivS]{\+F}$.
% We claim that for the syntactic semigroup $S$ of $(ab)^+$ over $\{a,b\}$,
% \[\Cl[\LocTrivS]{\+E}(S) \subsetneq \Cl[\LocTrivS]{\+F}(S).\]
% \todo{eggbox}
% Then $\Cl[\LocTrivS]{\+E}(S)$ consists of all singletons and of $\{0,ab\}$, $\{0, ba\}$.
% On the other hand, $\Cl[\LocTrivS]{\+F}(S)$ also contains $\{0,a\}$ since
% putting $x \defeq ab$, $y \defeq a$ and $z \defeq ba$ yields
% $x^{\idem} y z^{\idem} = a$ and $x^{\idem} z^{\idem} = 0$.

% \begin{corollary}
% 	$\LocTrivS$ is not "Henckell for $\+E$".
% \end{corollary}

==> sec/apdx-lifting-theorem-positive.tex <==
\section{Details on the Lifting Theorem for Positive Algebras}
\label{apdx:proof-thmlinftingsemigroups}


\subsection{Boolean Algebras \& Streams of Relations}
\label{apdx-proof:profinite-stream}

A \AP""profinite equivalence"" over variables $X$,
consists of a pair $(\type{u}{\sigma}, \type{v}{\tau}) \in \profSy{\SyncP X}$ denoted by \AP$u \intro*\profequiv v$.
A "relation" $\+R$ \AP""satisfies@@profequiv"" this "profinite equivalence"
when for all "positive synchronous algebra" $\?A$ recognizing $\+R$,
for all "morphism@@syncP" $\phi\colon \SyncP X \to \?A$,
$\profSy{\phi}(\type{u}{\sigma}) \in \phi[\+R] \Leftrightarrow
\profSy{\phi}(\type{v}{\tau}) \in \phi[\+R]$.

An \AP""explicit profinite equivalence"" ove the alphabet $\Sigma$
consists of a pair $(\type{u}{\sigma}, \type{v}{\tau}) \in \profSy{\SyncP \Sigma}$ also
denoted by \AP$u \profequiv v$. A "relation" $\+R$ over alphabet $\Sigma$ \AP""satisfies@@explprofequiv"" it when $u \in \bar{\+R}$ "iff" $v \in \bar{\+R}$.

\begin{proposition}
	\label{prop:reiterman-bool}
	Fix a finite alphabet $\Sigma$. A set of "synchronous relations"
	is a Boolean algebra if, and only if,
	it can be defined by a set of "explicit profinite equivalences" over $\Sigma$.
\end{proposition}

\begin{proof}
	The proof can be easily generalized from \cite[Theorem XII.2.6, p.~211]{pin_mathematical_2022}.
	One of the key argument is that if $\+R$ is "synchronous", then $\bar{\+R}$ is clopen in $\profSy{\SyncP \Sigma}$.
\end{proof}

A \AP""$+$-stream of relations"" consists of a map $\+V\colon \Sigma \mapsto \+V_\Sigma$
where each $\+V_\Sigma$ is a set of "relations" over $\Sigma$, such that:
\begin{itemize}
	\item $\+V_\Sigma$ is closed under Boolean operator,
	\item $\+V$ is closed under "inverse morphisms" of the form
		$\SyncP\Gamma \to \SyncP\Sigma$.
\end{itemize}

\begin{fact}
	\label{fact:equations-are-niiiice}
	Let $\+V$ be a "$+$-stream of relations", and $\Sigma$ be a finite alphabet.
	Then the following set coincides:
	\begin{itemize}
		\item $\+E^\Sigma_{\+V}$: the intersection of the set of all "profinite equivalences" satisfied by all relations of $\+V$, and of $\profSy{\SyncP \Sigma} \times \profSy{\SyncP \Sigma}$;
		\item $\+F^\Sigma_{\+V}$: the set of all "explicit profinite equivalences" satisfied by
		all relations of $\+V_{\Sigma}$.
	\end{itemize}
\end{fact}

\begin{proof}
	By construction, $\+E^\Sigma_{\+V} \subseteq \+F^\Sigma_{\+V}$. Conversely, let
	$(u \profequiv v) \in \+F^\Sigma_{\+V}$.
	To show that $(u \profequiv v) \in \+E^\Sigma_{\+V}$, we will show that all relations 
	$\+R \in \+V_{\Sigma}$ "satisfy@@profequiv" $u \profequiv v$, seen as a (non-explicit) "profinite dependency".
	So, let $\+R \in \+V_{\Sigma}$ and $\phi\colon \SyncP \Sigma \to \SyncP \Sigma$ be a "morphism@@syncP".
	Since $\+V$ is closed under preimages, $\phi^{-1}[\+R] \in \+V_{\Sigma}$.
	By continuity arguments, $\profSy{\phi}^{-1}[\bar{\+R}] = \phi^{-1}[\+R]$.
	Hence, $\profSy{\phi}(u) \in \bar{\+R}$ "iff" $u \in \profSy{\phi}^{-1}[\bar{\+R}] = \phi^{-1}[\+R]$. Since $\phi^{-1}[\+R] \in \+V_{\Sigma}$ satisfies the "explicit profinite equivalence"
	$u \profdep v$, it follows that $u \in \phi^{-1}[\+R] \Leftrightarrow v \in \phi^{-1}[\+R]$, and hence:
	\[
		\profSy{\phi}(u) \in \bar{\+R} \Leftrightarrow \profSy{\phi}(v) \in \bar{\+R}.
	\]
	This concludes the proof of $\+E^\Sigma_{\+V} \supseteq \+F^\Sigma_{\+V}$.
\end{proof}

We can then show an equivalent version of Reiterman's theorem for "streams".
This idea was introduced in the context of languages by Gehrke, Grigorieff and Pin, see
\cite[\S 8—9]{GGP08duality} or \cite[Theorem XIII.1.2, p.~224]{pin_mathematical_2022}.

\begin{proposition}[A Reiterman theorem for streams of relations]
	\label{prop:Reiterman-stream-relations}
	Let $\+V$ be a class of relations.
	$\+V$ is a "$+$-stream of relations" if, and only if, it is described
	by a set of "profinite equivalences".
\end{proposition}

\begin{proof}
	The right-to-left implication is easy and similar to the right-to-left
	implication of \Cref{thm:reiterman-sy}.
	
	So, let $\+V$ be a "$+$-stream of relations".
	Let $\+E$ be the set of all "profinite dependencies" "satisfied@@profdep" by
	$\+V$. Clearly, $\+V \subseteq \semprofdep{\+E}$.
	Conversely, let $\+R \in \semprofdep{\+E}$. Let $\Sigma$ be the alphabet over which $\+R$ is 
	written. By \Cref{fact:equations-are-niiiice}, $\+R$ satisfies all "explicit profinite 
	equivalences" satisfied by all "relations" of $\+V_{\Sigma}$.
	It follows from \Cref{prop:reiterman-bool} that $\+R \in \+V_{\Sigma}$.
\end{proof}

\begin{fact}
	\label{fact:Vrelations-is-stream}
	For any "$+$-pseudovariety of regular languages" $\+V$,\footnote{Of course the assumption can
	be weakened to $\+V$ being a stream.} "$\+V$-relations"
	form a "$+$-stream of relations".
\end{fact}

\begin{proof}
	Closure under Boolean operations follows from the closure under Boolean operations of $\+V$.
	Similarly, if $\phi\colon \SyncP\Gamma \to \SyncP\Sigma$ is a "morphism@@syncP"
	and $\+R \in \+V_\Sigma$, then let 
	$L \in \+V_{\Sigma}$ be such that $\+R = L \cap \WellFormed[\Sigma]$.
	Define $\psi\colon (\SigmaPair[\Gamma])^+ \to (\SigmaPair)^+$ by
	$\psi(\vec a) \defeq \phi(\vec a)$.
	Then
	\[\phi^{-1}[\+R] = \psi^{-1}[L] \cap \WellFormed[\Gamma].\]
	Since $\+V$ is closed by "inverse morphisms", $\psi^{-1}[L] \in \+V_{\Gamma}$
	and it follows that $\phi^{-1}[\+R]$ is a "$\+V$-relation".
\end{proof}

\subsection{Proof of the Lifting Theorem for Positive Semigroups}
\lemlinftingsemigroups*

\begin{fact}
	\label{fact:profequiv-pseudovar}
	Let $\+V$ be a "$+$-pseudovariety of regular languages". Let $u,v \in \profSg{X^+}$.
	The pseudovariety $\+V$ satisfies $u \profimp v$ "iff" it satisfies $u \profeq v$.
\end{fact}

\begin{proof}
	First, $\+V$ satisfies $u \profeq v$ "iff" it satisfies\footnote{This is because we are dealing with "$+$-pseudovarieties@@lang" and hence variables are interpreted as non-emtpy words.}
	\[
		u \profequiv v,\quad
		xu \profequiv xv,\quad
		uy \profequiv vy,\quad\text{and}\quad
		xuy \profequiv xvy,	
	\]
	where $x,y$ are new letters not occurring in $u$ or $v$.
	Then, we will show that $\+V$ satisfies $xuy \profequiv xvy$, the other cases being similar.
	Let $\Sigma$ be an alphabet and $L \in \+V_{\Sigma}$. Let $X$ be the set of variables of $u$ and $v$, and $\bar X \defeq X \cup \{x,y\}$. Let $S$ be the syntactic semigroup of $L$,
	and let $\phi\colon {\bar X}^+ \to S$ be a semigroup morphism.
	We want to show that $\profSg{\phi}(xuy) \in \phi[L]$ "iff" $\profSg{\phi}(xvy) \in \phi[L]$.
	Let $\Acc \defeq \profSg{\phi}(x)^{-1} \phi[L] \profSg{\phi}(y)^{-1}$.
	Denote by $\phi_X$ the restriction of $\phi$ to $X^+$.
	Since $\+V$ is a "$+$-pseudovariety@@lang", $\phi_X^{-1}[\Acc] \in \+V_{\Sigma}$,
	and hence it satisfies $u \profeq v$.
	It follows that $\profSg{\phi}(u) = \profSg{\phi_X}(u) \in \Acc$ "iff"
	$\profSg{\phi}(v) = \profSg{\phi_X}(v) \in \Acc$, and so, by definition of $\Acc$,
	$\profSg{\phi}(xuy) \in \phi[L]$ "iff" $\profSg{\phi}(xvy) \in \phi[L]$.
	Hence, $L$ satisfies $xuy \profequiv xvy$.
\end{proof}

\begin{proof}[Proof of \Cref{thm:lifting-semigroup}]\leavevmode
	\proofcase{$(1) \Rightarrow (2)$.}
	If $\+R$ is a "$\+V$-relation", then there exists a semigroup $S \in \B{V}$
	together with a semigroup morphism $\phi\colon (\SigmaPair)^+ \to S$
	such that $\+R = \phi^{-1}[\Acc] \cap \WellFormed$ for some $\Acc \subseteq S$.
	Consider the morphism it "induces@@syncP", namely
	\[
		\inducedmorSg{\phi}\colon \SyncP\Sigma \to \inducedalgSg{S}.	
	\]
	Then $\inducedmorSg{\phi}^{-1}[\Acc'] =
	\projP{\+R}$ where $\Acc'$ is the "closed subset" $\{\type{x}{\sigma} \mid x \in \Acc \land \sigma \in \types\}$ and so $\phi$ "recognizes@@sync" $\+R$.
	
	Moreover, we claim that $\inducedalgSg{S}$ satisfies all "profinite dependencies" of $\inducedProfdep{\EqVar{\B{V}}}$. Pick any $(u \profeq v) \in \EqVar{\B{V}}$, and let
	$\typing$ be a "typing consistent" with both "profinite words" $u$ and $v$. Fix a
	"morphism@@syncP" $\psi\colon \SyncP{X^{\typing}} \to \inducedalgSg{S}$, where $X$ denotes the set of
	variables of the "profinite equality" $u \profeq v$. We must show that
	$\profSy{\psi}(\substitProf{u}) \dep \profSy{\psi}(\substitProf{v})$.

	Consider the ``untyped'' version of $\psi$, $\psi_{\textsf{u}}\colon X^+ \to S$.
	Then $\profSg{\psi_{\textsf{u}}}(u) = \profSg{\psi_{\textsf{u}}}(v)$.
	It is then routine to check that $\profSy{\psi}(\substitProf{u}) =
	\type{(\profSg{\psi_{\textsf{u}}}(u))}{\sigma}$ where $\sigma$ is the "type" of
	$\substitProf{u}$, and similarly,
	$\profSy{\psi}(\substitProf{v}) =
	\type{\profSg{\psi_{\textsf{u}}}(v)}{\tau}$ where $\tau$ is the "type"
	of $\substitProf{v}$. Hence, from $\profSg{\psi_{\textsf{u}}}(u) = \profSg{\psi_{\textsf{u}}}(v)$ in $S$, it follows that
	$\profSy{\psi}(\substitProf{u}) \dep \profSy{\psi}(\substitProf{v})$ in
	$\inducedalgSg{S}$, which concludes the proof that 
	$\inducedalgSg{S}$ satisfies the "profinite dependency"
	$\substitProf{u} \profdep \substitProf{v}$.

	\proofcase{$(2) \Leftrightarrow (3)$.} Indeed, $\semprofdep{\inducedProfdep{\EqVar{\B{V}}}}$
	is a "pseudovariety of positive synchronous algebras".

	\proofcase{$(3) \Rightarrow (1)$.} This implication
	is quite surprising because its proof is not constructive---one could except
	the proof to explicitly build a semigroup $S$ accepting a language $L$
	such that $\+R = L \cap \WellFormed$ from $\SyntSAP{\+R}$.
	Since "$\+V$-relations" form a "$+$-stream of relations" by
	\Cref{fact:Vrelations-is-stream},
	they can be defined by a set of "profinite equivalences" by
	\Cref{prop:Reiterman-stream-relations}.
	Let $\+F$ be the set of all "profinite equivalences" "satisfied@@profequiv"
	by "$\+V$-relations".

	\begin{fact}
		\label{fact:no-more-equations}
		Let $u,v \in \profSy{\SyncP\Sigma}$.
		Define $u^{\?f}$ as the "profinite word" of $\profSg{(\SigmaPair)^+}$
		obtained from $u$ by forgetting the "types" of variables.
		If $u^{\?f} \profeq v^{\?f} \not\in \EqVar{\B{V}}$ then
		$(u \profequiv v) \not\in \+F$.
	\end{fact}
	Assume that $u^{\?f} \profeq v^{\?f} \not\in \EqVar{\B{V}}$. 
	Then by \Cref{fact:profequiv-pseudovar}, $\+V$ does not satisfy
	$u^{\?f} \profequiv v^{\?f}$.
	Let $\Sigma$ and $L \in \+V_\Sigma$ be such that
	$L$ does not satisfy $u^{\?f} \profequiv v^{\?f}$.

	To show $(u \profequiv v) \not\in \+F$, 
	it suffices then to build a "$\+V$-relation" $\+R_L$ whose
	"syntactic positive synchronous algebra" does not satisfy $u \profequiv v$.
	Let $\Gamma$ be any alphabet big enough so that $|\Gamma| \geq |\Sigma|$, and let
	$\mu$ be a collection of three surjective maps $\Gamma \times \Gamma \surj \Sigma$,
	$\Gamma \times \{\pad\} \surj \Sigma$ and $\{\pad\} \times \Gamma \surj \Sigma$.
	This naturally extends to a morphism $\mu\colon (\SigmaPair[\Gamma])^+ \to \Sigma^+$,
	and define $\+R$ as $\mu^{-1}[L] \cap \WellFormed[\Gamma]$. Since $\+V$ is a
	"$+$-pseudovariety of regular languages", $\mu^{-1}[L] \in \+V_\Gamma$ and hence $\+R$ is a "$\+V$-relation".
	By construction, for any $\type{w}{\sigma} \in \SyncP\Gamma$:
	\begin{equation}
		\type{w}{\sigma} \in \+R 
		\text{ "iff" }
		\mu(\type{w}{\sigma}) \in L.
	\end{equation}
	By continuity of $\profSg{\mu}$, and since $\bar L$ is clopen in $\profSg{\Sigma^+}$
	and $\bar{\+R}$ is clopen in $\profSy{\SyncP\Gamma}$---the proof of this claim can
	be easily adapted from \cite[Proposition X.3.16, p.~186]{pin_mathematical_2022}---,
	it follows that for all $\type{w}{\sigma} \in \profSy{\SyncP\Gamma}$:
	\[
		\type{w}{\sigma} \in \bar{\+R} 
		\text{ "iff" }
		\profSg{\mu}(\type{w}{\sigma}) \in \bar L.
		\label{eq:relationship-congruences-sgp-syncalg}
		\tag{\adforn{61}}
	\]

	By construction, $L$ does not satisfy $u^{\?f} \profequiv v^{\?f}$,
	so there exists a semigroup morphism $\phi\colon (X^{\?f})^+ \to \Sigma^+$---where
	$X$ is the set of variables of $u$ and $v$---such that $\profSg{\phi}(u^{\?f})
	\in \bar L$ but $\profSg{\phi}(v^{\?f}) \not\in \bar L$, or symmetrically.
	Pick any map $\psi\colon \SyncP X \to \SyncP\Gamma$ such that
	\[
		\profSy{\mu \circ \psi}(u) = \profSg{\phi}(u^{\?f}) \;\text{and}\;
		\profSy{\mu \circ \psi}(v) = \profSg{\phi}(v^{\?f}).
	\]
	Such a map must exist by construction of $\Gamma$ and $\mu$.
	Indeed, for $x \in X$, consider the word $\phi(x^{\?f}) \in \Sigma^+$.
	Recall---see \Cref{thm:reiterman-sy}---that "wlog" all variables of $X$ have type $\ll$ or
	$\lb$ or $\bl$. Assume "eg" that $x$ has type $\lb$ (the other cases are similar), 
	then since $\mu\colon \Gamma \times \{\pad\} \surj \Sigma$ is surjective, there
	exists $u \in (\Gamma\times\{\pad\})^+$, or equivalently $\type{u}{\lb} \in \SyncP\Gamma$,
	such that $\mu(u) = \phi(x^{\?f})$. Letting $\psi(\type{x}{\lb}) \defeq \type{u}{\lb}$
	defines a morphism $\psi\colon \SyncP X \to \SyncP\Gamma$ which satisfies the desired property.

	From $\profSg{\phi}(u^{\?f}) \in \bar L$ and $\profSg{\phi}(v^{\?f}) \not\in \bar L$,
	it follows by \eqref{eq:relationship-congruences-sgp-syncalg} that
	$\profSy{\psi}(u) \in \bar{\+R}$ but $\profSy{\psi}(v) \not\in \bar{\+R}$.
	Hence, the "$\+V$-relation" $\+R$ does not satisfy $u \profequiv v$.
	Therefore, $(u \profequiv v) \not\in \+F$, which concludes
	the proof of \Cref{fact:no-more-equations}.

	By $(1) \Rightarrow (3)$, $\inducedProfdep{\EqVar{\B{V}}} \subseteq \+F$,
	in the sense that for each $u \profequiv v$, then all four equations
	\[
		u \profequiv v,\quad
		xu \profequiv xv,\quad
		uy \profequiv vy,\quad\text{and}\quad
		xuy \profequiv xvy	
	\]
	belong to $\+F$.
	By the contraposition of \Cref{fact:no-more-equations}, if
	$(u \profequiv v) \in \+F$, then $u^{\?f} \profeq v^{\?f} \in \EqVar{\B{V}}$,
	which implies $(u \profdep v) \in \inducedProfdep{\EqVar{\B{V}}}$
	and by $(1) \Rightarrow (3)$, $(u \profdep v) \in \+F$.

	Let $\+F_0$ be the subset of "profinite dependencies" of $\+F$.
	By the paragraph above, a relation "satisfies@@profdep" $\+F$ "iff" it "satisfies@@profdep"
	$\+F_0$, and so, by definition of $\+F$:
	\begin{equation}
	\text{a relation is a "$\+V$-relation" "iff" it satisfies $\+F_0$.}
	\tag{\adforn{67}}
	\label{eq:equations-v-rel}
	\end{equation}

	We claim that $\inducedProfdep{\EqVar{\B{V}}} \supseteq \+F_0$.
	If $(u \profdep v) \in \+F_0$ then
	$(u^{\?f} \profeq v^{\?f}) \in \EqVar{\B{V}}$ by \Cref{fact:no-more-equations}, and so $(u \profdep v) \in \inducedProfdep{\EqVar{\B{V}}}$. Hence, if $\+R$ satisfies all "profinite dependencies" of $\inducedProfdep{\EqVar{\B{V}}}$, then it satisfies all "profinite dependencies" of $\+F_0$ and hence 
	by \eqref{eq:equations-v-rel}, it is a "$\+V$-relation". This concludes
	the proof of $(3) \Rightarrow (1)$.
\end{proof}

==> sec/apdx-positive-stuff.tex <==
\section{Details on Positive Synchronous Algebras}

\subsection{Composition of Algebras}
\label{apdx:sec:composition}

While the formal definition of the composition is quite different,
it is somehow conceptually similar to
Schützenberger's product---introduced in \cite[\adfS 2]{schutzenberger_finite_1965}, see also
\cite[\adfS 1]{straubing_generalization_1981} for a modern presentation---in the sense that
is relies on a powerset construction to simulate existential quantification.

The main idea is that, given $f\colon \SyncP\Sigma \to \?A$ and $g\colon \SyncP\Sigma \to \?B$,
when we will define $h\colon \SyncP\Sigma \to \?A\compos\?B$, which will recognize any composition\footnote{We chose the natural, and hence non-standard, definition, namely $\+R \circ \+S$ is the set of pairs $(u,w)$ "st" $(u,v) \in \+R$ and $(v,w) \in \+S$ for some $v$.}
of a relation recognized by $f$ and by $g$, we must encode in $h\pair{u}{w}$ the 
set of possible values $\big( f\pair{u}{v}, g\pair{v}{w} \big)$, when $v$ ranges over finite words.

\begin{definition}[Composition]
	Given two "positive synchronous algebras" $\?A$ and $\?B$, define their composition 
	$\?A \intro*\compos \?B$ as the algebra $\?C$ where:
	\begin{itemize}
		\item $C_{\sfrac{a}{b}\to\sfrac{c}{d}} = \pset\bigl(\bigcup_{e,f \in \{l,b\}} A_{\sfrac{a}{e}\to \sfrac{c}{f}}
		\times B_{\sfrac{e}{b}\to \sfrac{f}{d}}\bigr)$ for all $\sfrac{a}{b}\to\sfrac{c}{d} \in \types$;
		\item the product of $\type{X}{\tau} \in \?C$ with $\type{X'}{\tau'} \in \?C$ is defined  
			as
			\begin{align*}
			\type{\big\{
				\langle\type{(x\cdot x')}{\rho\concattype \rho'}, \type{(y\cdot y')}{\sigma\concattype \sigma'}\rangle
					\;\big\vert\; & (\type{x}{\rho}, \type{y}{\sigma}) \in \type{X}{\tau},\;
					(\type{x'}{\rho'}, \type{y'}{\sigma'}) \in \type{X'}{\tau'} \\
				& \text{ and both $(\rho, \rho')$ and $(\sigma,\sigma')$ are "compatible"}
				\big\}}{
				\tau\concattype\tau'
			}
			;\end{align*}
		\item the "dependency relation" is equality.
	\end{itemize}
\end{definition}

\begin{fact}
	If two relations $\+R$ and $\+S$ are "recognized@@sync" by $\?A$ and $\?B$, respectively,
	then $\+R \circ \+S$ is "recognized@@sync" by $\?A\compos \?B$.
\end{fact}

\begin{proof}[Proof sketch]
	Say that $\phi\colon \SyncP\Sigma \to \?A$ "recognizes@@sync" $\+R$ and
	$\psi\colon \SyncP\Sigma \to \?B$ "recognizes@@sync" $\+S$.
	Then we define $\chi\colon \Sync\Sigma \to \?A \compos \?B$ as follows:
	for each pair $\type{(u,w)}{\sfrac{a}{b}\to\sfrac{c}{d}} \in \Sync\Sigma$,
	$\chi(\type{(u,w)}{\sfrac{a}{b}\to\sfrac{c}{d}})$ is defined as the "closed subset"
	\[
		\bigl\{\langle\phi(\type{(u,v)}{\sfrac{a}{e}\to \sfrac{c}{f}}),
		\,\psi(\type{(v,w)}{\sfrac{e}{b}\to \sfrac{f}{d}})\rangle
		\;\big\vert\;
		v \in \Sigma^* \text{ and }
		\type{(u,v)}{\sfrac{a}{e}\to \sfrac{c}{f}}, \type{(v,w)}{\sfrac{e}{b}\to \sfrac{f}{d}} \in \Sync\Sigma \bigr\}.
	\]
	Then $\+R \circ \+S$ is the preimage by $\chi$ of the set of all subsets
	containing a pair $\langle a, b \rangle \in \?A \times \?B$
	"st" $a\in \phi[\proj{\+R}]$ and $b \in \psi[\proj{\+S}]$.
\end{proof}

\subsection{Canonicity of the Consolidation of the Syntactic Positive Synchronous Algebra Morphism}
\label{apdx:canonicity-consolidation}

We formalize the idea that $\consolSyntSAP{\+R}$ is the \emph{canonical}
and \emph{minimal} (in an algebraic sense, as usual) semigroup
"recognizing@@sync" $\+R$ that can be typed.

\begin{proposition}
	\label{prop:cartesian-product-morphisms}
	For any semigroup $T$ together with surjective semigroup morphisms
	\[
		\phi\colon (\SigmaPair)^+ \surj T,
		\quad
		\rho_{\text{type}}\colon T \surj \consol{\?1}
		\quad\text{ and }\quad
		\rho_{\text{val}}\colon T \surj S_{\+R}
	\]
	such that $\rho_{\text{type}}\circ \phi = \text{type}$ and
	$\rho_{\text{val}}\circ \phi = \zeta_{\+R}$, there exists a semigroup morphism
	$\psi\colon T \surj \consolSyntSAP{\+R}$ such that 
	$\sgpSyntSAMP{\+R} = \psi \circ \phi$.
	In other words, the following diagram commutes:
	\begin{center}
		\begin{tikzcd}[row sep=scriptsize, every arrow/.append style={two heads}]
			&
			% Top node
			(\SigmaPair)^+
				\ar[d, "\phi", pos=.65]
				\ar[ddl, "\typemap" swap]
				\ar[ddr, "\zeta_{\+R}"]
			& \\[2.5em]
			&
			% Background node
			|[xshift=.3cm]| T
				\ar[dl, "\rho_{\text{type}}" swap, pos=.3]
				\ar[dr, "\rho_{\text{val}}", pos=.1]
				\ar[from=1-2, to=4-2, "\sgpSyntSAMP{\+R}" swap, pos=.35, crossing over]
				\ar[dd, "\psi", dashed]
			& \\[-.5em]
			% Left node
			|[yshift=.2cm]| \consol{\?1}
			& &
			% Right node
			|[yshift=-.2cm]| S_{\+R}.
			\\[-.5em]
			&
			% Foreground node
			|[xshift=-.3cm]| \consolSyntSAP{\+R}
				\ar[ul, "\projtype"]
				\ar[ur, "\projval" swap]
			&
		\end{tikzcd}
	\end{center}
\end{proposition}

The previous proposition can be nicely reformulated in categorical terms:
denote by $(\SigmaPair)^+ \coslicesurj \cat{Sgp}$ the full subcategory of
the "coslice category" $(\SigmaPair)^+ \coslice \cat{Sgp}$ induced by surjective morphisms,
"ie" it is the category whose objects are surjective semigroup morphisms $\phi\colon (\SigmaPair)^+ \surj T$,
and whose morphisms from $\phi\colon (\SigmaPair)^+ \surj T$ to $\psi\colon (\SigmaPair)^+ \surj U$
are simply the semigroup morphisms $\chi\colon T \to U$ such that $\psi = \chi \circ \phi$.
Then the syntactic semigroup morphism of "well-formed words" (namely $\typemap$)
and of $\+R$, seen as objects of $(\SigmaPair)^+ \coslicesurj \cat{Sgp}$,
admit a "Cartesian product@@cat", and this product is the composition
$\sgpSyntSAMP{\+R}\colon (\SigmaPair)^+ \surj \consolSyntSAP{\+R}$ of the
of the "consolidation" of the "syntactic synchronous morphism" of $\+R$
together with the canonical surjection $\sigma\colon (\SigmaPair)^+ \surj \consol{(\Sync\Sigma)}$.

% \todo{proof!!}

\begin{remark}
	Finally, note that this property implies that if $\consol{\?1} \in \B{V}$, then
	$\consolSyntSAP{\+R} \in \B{V}$ "iff" $S_{\+R} \in \B{V}$.
	Indeed, if $\consolSyntSAP{\+R} \in \B{V}$, then, as a "quotient@@sync",
	$S_{\+R} \in \B{V}$.
	Conversely, if $S_{\+R} \in \B{V}$ then $S_{\+R} \times \consol{\?1} \in \B{V}$ since
	$\consol{\?1} \in \B{V}$, and since 
	$S_{\+R} \times \consol{\?1}$ comes naturally equipped with projections
	onto $S_{\+R}$ and $\consol{\?1}$, by \Cref{prop:cartesian-product-morphisms},
	$\consolSyntSAP{\+R}$ is a "quotient@@sync" of $S_{\+R} \times \consol{\?1}$
	and hence belongs to $\B{V}$.
	This statement is the algebraic counterpart of \Cref{fact:a-triviality-on-trivial-relations}.
\end{remark}


\subsection{Profinite Topology \& Pseudovarieties}
\label{apdx-proof:profinite-pseudovar}

For any "pseudovariety of positive synchronous algebras" $\B{V}$, let
\AP\phantomintro{\distvar}\phantomintro{\ristvar}
\begin{align*}
	\reintro*\distvar(u,v) & \defeq 2^{-\ristvar(u,v)} \text{ where } \\
	\reintro*\ristvar(u,v) & \defeq 
	\min{\bigl\{n\in \N \mid}
	\text{ $\phi(u) \not\dep \phi(v)$ for some "morphism@@syncP"} \\[-.2em]
	& \hphantom{\defeq \min{\bigl\{n\in \N \mid}}
		\text{ $\phi$ whose codomain has at most} \\[-.35em]
	& \hphantom{\defeq \min{\bigl\{n\in \N \mid}}
		\text{ $n$ elements and is in $\B{V}$.}\bigr\}.
\end{align*}
Then define the "congruence@@sync" \AP$\intro*\simvar$ over $\profSy{\SyncP \Sigma}$
by $u \simvar v$ "iff" $\distvar(u,v) = 0$.
Then $\intro*\freepro\Sigma \defeq \profSy{\SyncP\Sigma}/{\simvar}$
is a "positive synchronous algebra", called
the \AP""free pro-$\B{V}$ positive synchronous algebra"".

Note however that contrary to the free pro-$\B{V}$
semigroup---see \cite[\S XI.2, p.~190]{pin_mathematical_2022}---it
is not a compact metric space, for the simple reason that one can have $\distvar(u,v) = 0$
for some $u \neq v \in \profSy{\SyncP\Sigma}/{\simvar}$ of different type.
However, the "free pro-$\B{V}$ positive synchronous algebra"
is a compact ultrapseudometric space, and all restrictions
of $\profSy{\SyncP\Sigma}/{\simvar}$ are metric ("aka" $T_0$).
Most properties of metric space can easily be generalized to pseudometric spaces,
see "eg" \cite[Theorem 17.33, p.~470]{schechter1996handbook} for a characterization of
compactness.

Sending a "profinite word" to its equivalence class under $\simvar$
defines a canonical surjective morphism
\[\AP\intro*\freeproproj\colon\profSy{\SyncP \Sigma} \surj \freepro\Sigma\]
which happens to be 1-Lipschitz and hence uniformly continuous.

\begin{proposition}
	\label{prop:free-proV-extension-morphism}
	Every "morphism@@syncP" $\phi\colon \SyncP\Sigma \to \?A$ where $\?A \in \B{V}$
	extends to a unique uniformly continuous morphism $\freepro\Sigma \to \?A$.
\end{proposition}

\begin{proof}
	Similar to \cite[Proposition XI.2.6, p.~192]{pin_mathematical_2022}.
\end{proof}

\begin{proposition}
	\label{prop:continuous-quotient}
	A finite $\SigmaPair$-generated "algebra@@syncP" belongs to $\B{V}$
	if and only if it is a continuous quotient of $\freepro\Sigma$,
	is the sense that it is the image of $\freepro\Sigma$ by a continuous "morphism@@syncP".
\end{proposition}

\begin{proof}
	Similar to \cite[Proposition XI.2.7, p.~192]{pin_mathematical_2022}.
\end{proof}

\begin{proposition}
	\label{prop:equations-vs-free-proV}
	Let $u,v \in \profSy{\SyncP X}$. Then all "algebras@@syncP" of $\B{V}$
	"satisfy@@profdep" $u \profdep v$ "iff" $\freeproproj(u) \dep \freeproproj(v)$.
\end{proposition}

\begin{proof}
	Similar to \cite[Proposition XI.3.11, p.~195]{pin_mathematical_2022}.
\end{proof}

\lemmareiterman*

\begin{proof}[Proof of \Cref{thm:reiterman-sy}]
	We follow the proof of \cite[Theorem XI.3.13, p.~195]{pin_mathematical_2022}.

	\proofcase{Converse implication.} Let $\+E$ be a set of "profinite dependencies".
	Let us show that $\semprofdep{\+E}$ is a "pseudovariety of positive synchronous algebras".
	Let $\?A_1, \?A_2 \in \semprofdep{\+E}$. For any $(\type{u}{\sigma} \profdep \type{v}{\tau}) \in
	\+E$, let $X$ be its set of variables. Then for every "morphism@@syncP" $\phi\colon \SyncP X \to \?A_1 \times \?A_2$, let $\pi_1, \pi_2$ be the canonical projection from $\?A_1\times \?A_2$
	to $\?A_1$ and $\?A_2$, respectively. Then $\pi_i \circ \phi$ is a "morphism@@syncP"
	$\SyncP X \to \?A_i$ and hence
	$\profSy{\pi_i \circ \phi}(\type{u}{\sigma}) \dep^{\?A_i} \profSy{\pi_i \circ \phi}(\type{v}{\tau})$.
	From $\profSy{\pi_i \circ \phi} = \pi_i \circ \profSy{\phi}$ it follows that
	\begin{align*}
		\profSy{\phi}(\type{u}{\sigma}) =
		\langle \profSy{\pi_1 \circ \phi}(\type{u}{\sigma}), \,
			\profSy{\pi_2 \circ \phi}(\type{u}{\sigma}) \rangle
		&  \\
		& \hspace{-2cm} \dep^{\?A_1\times\?A_2} \langle \profSy{\pi_1 \circ \phi}(\type{v}{\tau}), \,
			\profSy{\pi_2 \circ \phi}(\type{v}{\tau}) \rangle
		= \profSy{\phi}(\type{v}{\tau}).
	\end{align*}
	Hence $\?A_1\times\?A_2 \in \semprofdep{\+E}$.
	Observe then that $\semprofdep{\+E}$ is obviously closed under
	"subalgebras". For quotients, let $\?A \in \semprofdep{\+E}$,
	and consider a "quotient@@sync" $\psi\colon \?A \surj \quotient{\?A}{\asympbar}$.
	Then for every "profinite dependency" $u \profdep v$ over $X$,
	for every $\phi\colon \SyncP X \to \quotient{\?A}{\asympbar}$,
	then there exists $\chi\colon \SyncP X \to \?A$ "st" $\phi = \psi \circ \chi$.\footnote{Map
	$x \in X$ to any element $a \in \?A$ "st" $\phi(x) = \equivclass{a}{\asympbar}$. Such an element
	must exist by surjectivity of $\psi$.} And hence, from $\profSy{\psi \circ \chi} = \psi \circ \profSy{\chi}$, it follows that
	\[
		\profSy{\phi}(\type{u}{\sigma}) = \psi(\profSy{\chi}(\type{u}{\sigma}))	
		\dep \psi(\profSy{\chi}(\type{v}{\tau})) = \profSy{\phi}(\type{v}{\tau}).
	\]

	\proofcase{Direct implication.} Let $\+E$ be the set of "profinite dependencies satisfied"
	by all "algebras@@syncP" of $\B{V}$. Let $\B{W} \defeq \semprofdep{\+E}$.
	By the previous implication, it is a "pseudovariety of positive synchronous algebras", and
	by construction $\B{V} \subseteq \B{W}$. We want to show the converse inclusion, so let $\?A \in \B{W}$. Since $\?A$ is finite and "locally generated", there exists
	a finite alphabet $\Sigma$ and a surjective "morphism@@syncP"
	$\phi\colon \SyncP\Sigma \surj \?A$. It induces a uniformly continuous "morphism@@syncP"
	$\profSy{\phi}\colon \profSy{\SyncP\Sigma} \surj \?A$. Pick $u,v \in \profSy{\SyncP\Sigma}$.
	Observe that if $\freeproproj(u) \dep \freeproproj(v)$ then by \Cref{prop:equations-vs-free-proV},
	$u \profdep v$ is "satisfied@@profdep" by all "algebras@@syncP" in $\B{V}$
	and hence belongs to $\+E$. Hence, $\?A$ satisfies $u \profdep v$, and thus
	$\profSy{\phi}(u) \dep \profSy{\phi}(v)$. By second isomorphism theorem, it follows
	that there exists a "morphism@@syncP" $\gamma\colon \freepro\Sigma \surj \?A$ such that
	$\profSy{\phi} = \gamma \circ \freeproproj$.
	
	We then claim that $\gamma$ is continuous. Indeed, $\?A$ is discrete, and for each $\type{x}{\sigma}$, $\gamma^{-1}[\type{x}{\sigma}] = \freeproproj[\B{V}][\profSy{\phi}^{-1}[\type{x}{\sigma}]]$.
	By continuity of $\profSy{\phi}$, $\profSy{\phi}^{-1}[\type{x}{\sigma}]$ is closed (in fact clopen),
	and hence compact as a closed subset of the compact space $\profSy{\SyncP\Sigma}$.
	Then $\freeproproj[\B{V}][\profSy{\phi}^{-1}[\type{x}{\sigma}]]$ is compact, as the image of a
	compact set by a continuous map, and hence in particular it is closed.

	Therefore, $\gamma$ is a continuous morphism, proving that $\?A$ is a continuous quotient
	of $\freepro\Sigma$. Hence, by \Cref{prop:continuous-quotient}, $\?A \in \B{V}$which concludes the proof that $\B{V} = \B{W}$.
\end{proof}


==> sec/lifting-theorem-positive.tex <==
\section{The Lifting Theorem for Positive Algebras}
\label{sec:lifting-theorem-semigroups}

\subsection{Some Examples}

In most of this section,
we fix an "Eilenberg-Schützenberger correspondence@@Sg" $\+V \corr \B{V}$ between
a "$+$-pseudovariety of regular languages" and a "pseudovariety of semigroups".

In \Cref{ex:counter-ex-group-relations-semigroups}, we showed that not all "relations" 
whose "syntactic positive synchronous algebra" whose "underlying semigroups"
are all groups are necessarily "group relations". In fact, it is quite easy
to find a necessary and sufficient condition on the "syntactic positive algebra@@sync"
to characterize "group relations".

\begin{example}[Group relations: \Cref{ex:counter-ex-group-relations-semigroups}, cont'd]
	\label{ex:charac-group-relations-semigroups}
	Let $\+R \subseteq (\Sigma^* \times \Sigma^*) \smallsetminus \{(\varepsilon, \varepsilon)\}$. Then $\+R$ is a "group relation" if and only if it is "recognized@@sync"
	by a finite "positive synchronous algebra" $\?A$ such that:
	\begin{itemize}
		\item every "underlying semigroup" of $\?A$ is a group, and moreover
		\item for each $\type{1}{\sigma}, \type{x}{\tau} \in \?A$,
			$\type{1}{\sigma}\cdot \type{x}{\tau} \dep \type{x}{\tau}$
			if $\sigma, \tau$ are "compatible" and 
			$\type{x}{\tau}\cdot \type{1}{\sigma} \dep \type{x}{\tau}$
			if $\tau, \sigma$ are "compatible", where $\type{1}{\sigma}$ is the unit of "type" 
			$\sigma$.
	\end{itemize}
	The left-to-right implication follows from the construction of the "positive synchronous algebra induced" by a semigroup.~The right-to-left implication
	follows from the fact that $\?A$ must in fact be a "synchronous algebra"
	and \Cref{thm:lifting-theorem-monoids}.
\end{example}

Notice how the second item of this condition is an axiom of (non-positive) "synchronous algebras".

Interestingly, some "$\+V$-relations" can still be characterized by solely looking
at the "underlying semigroups" of their "syntactic positive synchronous algebra".

\begin{example}[Commutative relations]
	\label{ex:commutative-relations}
	Let $\+R \subseteq (\Sigma^* \times \Sigma^*) \smallsetminus \{(\varepsilon, \varepsilon)\}$. 
	Define \AP""commutative relations"" as the "$\+V$-relations" where $\+V$ is the
	class of commutative languages, "corresponding@@EilenbergSg" to the pseudovariety of commutative semigroups.
	Then $\+R$ is a "commutative relation" if and only if it is "recognized@@sync"
	by a finite "positive synchronous algebra" $\?A$ such that
	every "underlying semigroup" of $\?A$ is a commutative semigroup.
	The left-to-right implication is, as always, trivial, by
	considering the "positive synchronous algebra induced" by a semigroup.
	For the converse, let $S_{\ll}, S_{\lb}$ and $S_{\bl}$. Consider the
	\emph{unit adjunction} operation $-^1$, which consists of taking a semigroup
	and \emph{always} adding a unit to it, making it into a monoid.
	Then \[M \defeq S_{\ll}^1 \times S_{\lb}^1 \times S_{\bl}^1\] is a commutative semigroup,
	and recognizes $\+R$ as a subset of $(\SigmaPair)^+$, using the same
	construction as \Cref{thm:lifting-theorem-monoids}. Note that proving this
	must \emph{crucially} rely on the fact that the unit adjunction adds a new unit to
	every semigroup (even if the original semigroup already has a unit).
\end{example}

More generally, the construction above can be generalized with ease to any "pseudovariety of 
semigroups" closed under unit adjunction. For such classes, "$\+V$-relations" are exactly those
"recognized@@sync" by "positive synchronous algebras" whose "underlying semigroups" belong to
$\B{V}$. Both \Cref{ex:counter-ex-group-relations-semigroups,ex:commutative-relations} have the particularity to deal with "pseudovarieties@@semigroup" that particularly interact nicely with
units, and hence are not too different from the setting of \Cref{thm:lifting-theorem-monoids}.

A natural question is to then study classes which are intrinsically allergic to units: can
a nice characterization of "$\+V$-relations" be found in this case?

\begin{example}[Nilpotent relations: \Cref{ex:nilpotent}, cont'd]
	\label{ex:nilpotent-charac}
	A "relation" $\+R \subseteq (\Sigma^* \times \Sigma^*) \smallsetminus \{(\varepsilon, \varepsilon)\}$ is a ""$\Nil$-relation"" if, and only if, it is recognizing by
	a finite "positive synchronous algebra" $\?A$ such that:
	\begin{itemize}
		\item every "underlying semigroup" of $\?A$ is "nilpotent", and moreover
		\item for each $\type{0}{\sigma}, \type{x}{\tau} \in \?A$,
		$\type{0}{\sigma}\cdot \type{x}{\tau} \dep \type{0}{\sigma}$
		if $\sigma, \tau$ are "compatible" and 
		$\type{x}{\tau}\cdot \type{0}{\sigma} \dep \type{0}{\sigma}$
		if $\tau, \sigma$ are "compatible", where $\type{0}{\sigma}$ denotes
		either the zero of the "underlying semigroup" of type $\sigma$,
		if $\sigma \in \{\ll,\lb,\bl\}$, or $\type{0}{\ll}\cdot \type{0}{\beta}$
		for $\beta \in \{\lb,\bl\}$ if $\sigma = \ll \to \beta$.
	\end{itemize}
	To prove the converse implication, one can notice that any accepting set
	must either contain all zeroes of $\?A$, or none of them.
	In the former case, one can then show that the preimage of $\Acc$
	is finite, and in the latter set, its "complement@@rel" is finite.
	The conclusion follows from \Cref{ex:nilpotent}.
\end{example}

It turns out that the characterizations of
\Cref{ex:charac-group-relations-semigroups,ex:commutative-relations,ex:nilpotent-charac} can be described in a unified way using "profinite dependencies": the idea is to look at
some "profinite equalities"
defining $\B{V}$ (for instance $\{x^{\idem}y = y,\, y x^{\idem} = y\}$ for groups%,
% or $\{xy = yx\}$ for commutative semigroups
), and transform them into "profinite dependencies" 
by (a) non-deterministically guessing the "type" of the variables so that both sides of the equation are "well-typed", and (b) changing the equality symbol into a "dependency" symbol.
For instance, $x^{\idem}y = y$ gives rise, among others, to the "profinite dependencies"
$\type[\idem]{x}{\ll} \type{y}{\ll} \profdep \type{y}{\ll}$,
$\type[\idem]{x}{\ll} \type{y}{\lb} \profdep \type{y}{\lb}$
and $\type[\idem]{x}{\ll} \type{y}{\ll\to\lb} \profdep \type{y}{\ll\to\lb}$.
% On the other hand, for commutative
% relations, for both $\type{x}{\sigma}\type{y}{\tau}$ and $\type{y}{\tau}\type{x}{\sigma}$
% to be "well-typed", one needs to have $\sigma = \tau \in \{\ll,\lb,\bl\}$, and so
% $xy = yx$ exactly induces the three "profinite dependencies"
% \[
% 	\type{x}{\tau} \type{y}{\tau} = \type{y}{\tau} \type{x}{\tau},
% 	\quad \tau \in \{\ll,\lb,\bl\}.
% \]
It can then be checked that the characterization of \Cref{ex:charac-group-relations-semigroups,ex:commutative-relations,ex:nilpotent-charac} exactly corresponds to
the "profinite dependencies" induced by the profinite equalities
$\{x^{\idem}y = y,\, y x^{\idem} = y\}$ (for groups),
$\{xy = yx\}$ (for commutative semigroups), and
$\{x^{\idem}y = x^{\idem},\, y x^{\idem} = x^{\idem}\}$ (for "nilpotent semigroups"), respectively.

\subsection{Induced Profinite Dependencies \& the Lifting Theorem}

We now proceed to give a formal definition of the set of "profinite dependencies induced by a 
profinite equality". Given a set $X$, and a function \AP$\intro*\typing\colon X \to \types$
called \AP""typing"",
we denote by $X^{\typing}$ the "typed set" $\langle \typing^{-1}[\tau]\rangle_{\tau \in \types}$.
We say that $\tau$ is \AP""consistent@@typing"" with a word $u \in X^+$ if
the list of types $\langle \typing(u_i)\rangle_{i \in \dom(u)}$ is "compatible". We
say that $\tau$ is \reintro[typing]{consistent} with a "profinite word" $u = (u_n)_{n\in\N}$,
if there exists some $n_0\in\N$ such that for all $n \geq n_0$,
$\typing$ is "consistent@@typing" with word $u_n \in X^+$.
Clearly, if $\typing$ is "consistent@@typing" with word $u \in X^+$, then
the word \AP$\intro*\substitWord{u}$ obtained by replacing every letter $x$ by
the associated element in $X^{\typing}$ is an element of $\SyncP{X^{\typing}}$.
\begin{fact}
	If $\typing$ is "consistent@@typing" with two words $u, v \in X^+$, then
	the smallest semigroup separating $u$ and $v$
	is upper-bounded, up to an additive constant,
	by the size of the smallest "positive synchronous algebra"
	separating $\substitWord{u}$ and $\substitWord{v}$.\footnote{This result can be proven by
	considering the "consolidation".}
\end{fact}
It follows that if $\typing$ is "consistent@@typing" with a "profinite word"
$u$, say $(u_n)_{n\in\N} \in \profSg{X^+}$, then \AP$\intro*\substitProf{u} \defeq
(\substitWord{u_n})_{n\in\N}$ is "Cauchy" and hence belongs in $\profSy{\SyncP{X^{\typing}}}$.

\begin{definition}
	Given a "profinite equality" $u \profeq v$ over variables $X$, the \AP""profinite dependencies 
	induced by"" $u \profeq v$ is defined as the set of "profinite dependencies"
	\[
		\intro*\inducedProfdep{(u \profeq v)} \defeq
		\bigl\{
			\substitProf{u} \profdep \substitProf{v} \;\big\vert\;
			\typing \text{ is "consistent@@typing" with both $u$ and $v$}
		\bigr\}.
	\]
	We extend the notation additively to sets of equations.
\end{definition}

Then \Cref{ex:charac-group-relations-semigroups} can be reformulated as follows:
a "relation" is a "group relation" if, and only if, it is "recognized@@sync" by
a "positive synchronous algebra" which "satisfies@@profdep" all "profinite dependencies"
of $\inducedProfdep{\{x^{\idem}y = y,\, y x^{\idem} = y\}}$.

Remark that the "typing" $\typing\colon X \to \types$ that is always equal to $\sigma$,
for $\sigma \in \{\ll, \lb, \bl\}$, is always "consistent@@typing" with
any "profinite word". Also recall that $\type{x}{\sigma} \dep \type{y}{\sigma}$
always implies $\type{x}{\sigma} = \type{y}{\sigma}$.
\begin{fact}
	For any set $\+E$ of "profinite equalities" "defining@@profeq" $\B{V}$,
	if a finite "positive synchronous algebra" $\?A$ "satisfies@@profdep"
	all "profinite dependencies induced"
	by $\+E$, then all "underlying semigroups" of $\?A$ belong to $\B{V}$.
\end{fact}

Note that given a set $\+E$ of "profinite equalities" "defining@@profeq" $\B{V}$,
the class of all finite "locally generated" "positive synchronous algebras"
$\semprofdep{\inducedProfdep{\+E}}$---namely the "algebras@@syncP" "satisfying@@profdep"
all "profinite dependencies induced" by $\+E$---is a "pseudovariety of
positive synchronous algebras" as a consequence of \Cref{thm:reiterman-sy}.
In light of the examples presented above, it is quite natural to conjecture
that this is the class "corresponding@@EilenbergSy" to "$\+V$-relations".
We show that, somewhat surprisingly, the choice of $\+E$ matters.

\begin{example}[Locally trivial relations]
	\label{ex:locally-trivial-relations}
	The "pseudovariety of semigroups" "corresponding@@EilenbergSg" to
	$\LocTriv$ can be equivalently defined by the "profinite equality"
	$x^{\idem} y x^{\idem} = x^{\idem}$, or by
	$x^{\idem} y z^{\idem} = x^{\idem} z^{\idem}$, see
	\cite[Proposition XI.4.17, p.~197]{pin_mathematical_2022}.
	A relation is a "$\LocTriv$-relation" "iff"
	it is "recognized@@sync" by a finite "positive synchronous algebra"
	satisfying all "profinite dependencies induced" by
	$x^{\idem} y z^{\idem} = x^{\idem} z^{\idem}$.
	On the other hand, there are "relations" whose "syntactic positive synchronous algebra"
	satisfies all "profinite dependencies induced" by
	$x^{\idem} y x^{\idem} = x^{\idem}$, but which are not "$\LocTriv$-relations".
	% Details are given in \Cref{apdx:sec:locally-trivial-relations}.
	To intuitively grasp why
	\[\semprofdep{\inducedProfdep{(x^{\idem} y x^{\idem} = x^{\idem})}}
	\subsetneq \semprofdep{\inducedProfdep{(x^{\idem} y z^{\idem} = x^{\idem} z^{\idem})}}\]
	one can notice that there are much fewer "typings"
	"consistent@@typing" with $x^{\idem} y x^{\idem}$ than with
	$x^{\idem} y z^{\idem}$.
\end{example}

\Cref{ex:charac-group-relations-semigroups,ex:commutative-relations,ex:nilpotent-charac,ex:locally-trivial-relations} lead to the following result. \AP\phantomintro{\EqVar}
\phantomintro(semigroups){lifting theorem}
\thmlinftingsemigroups
See the proof in \Cref{apdx:proof-thmlinftingsemigroups}.

\begin{proof}[Proof sketch]
	Implications $(1) \Rightarrow (2) \Rightarrow (3)$ are relatively straightforward and
	similar to the proof of $(1) \Rightarrow (2) \Rightarrow (3)$ of
	\Cref{thm:lifting-theorem-monoids}.
	The interesting implication is $(3) \Rightarrow (1)$: we need to show
	that if the class of all "$\+V$-relations" satisfies some "profinite dependency"
	$u \profdep v$, then $\+V$ satisfies $u^{\?f} \profeq v^{\?f}$ where $u^{\?f}$
	and $v^{\?f}$ are obtained from $u$ and $v$ by forgetting the type of variables.
	Directly proving this is particularly hard because of the definition of "residuals".
	Our proof uses a generalization of profinite equations, namely
	"explicit profinite equivalence" introduced by Gehrke, Grigorieff \& Pin \cite[\S 8—9]{GGP08duality}---see
	\Cref{apdx-proof:profinite-stream}.
	Our main technical lemma shows that if
	"$\+V$-relations" "satisfy@@profequiv" an "explicit profinite equivalence"
	$u \profequiv v$, then $\+V$ "satisfy@@profequiv" $u^{\?f} \profequiv v^{\?f}$.
	We conclude using an adaptation of Reiterman theorem to streams (a generalisation of
	pseudovarieties, see \Cref{prop:Reiterman-stream-relations}).
\end{proof}

Note however \Cref{thm:lifting-semigroup} does not imply decidability: first, there are uncountably 
many "profinite words", and second, $\EqVar{\B{V}}$ is infinite. 
% We describe in \Cref{apdx:henckell} a sufficient condition for the set
% $\inducedProfdep{\EqVar{\B{V}}}$ to be equivalent to a finite
% set of "profinite dependencies", based on the theory of pointlike sets.

==> sec/positive-synchronous-algebras.tex <==
\section{Positive Synchronous Algebras}
\label{sec:positive-synchronous-algebras}

\subsection{Axiomatization}

The only drawback from \Cref{sec:synchronous-algebras,sec:lifting-theorem} is that
it deals with "$\ast$-pseudovarieties of regular languages", but many interesting classes
do not satisfy this property but only are "$+$-pseudovarieties of regular languages".\footnote{These
"$+$-pseudovarieties@@reglang" correspond to "pseudovarieties of semigroups". Crucially, note that
"pseudovarieties of semigroups" and of "finite monoids@pseudovarieties of monoids" do not only
differ by the presence of units: "pseudovarieties of semigroups" have slightly weaker
closure properties.}
This includes "e.g." the class $\Nil$.
or the class of
\emph{locally trivial languages}
\[
	\AP\intro*\LocTriv_{\Sigma} \defeq
	\{F \Sigma^* G \cup H \mid F, G, H \mathrel{\subseteq_{\textsf{finite}}} \Sigma^+\}.
\]
In this section, we introduce "positive synchronous algebras", which are essentially
"synchronous algebras" without the restriction to have units.

\begin{definition}
	A \AP""positive synchronous algebra"" $\langle \?A, \cdot, \dep \rangle$ consists of a "dependent set" $\langle \?A, \dep \rangle$ together
	with a partial binary operation $\cdot$ on $\?A$, called "product" such that:
	\begin{itemize}
		\item for $\type{x}{\sigma}, \type{y}{\tau} \in \?A$,
			$\type{x}{\sigma} \cdot \type{y}{\tau}$ is defined "iff" $\sigma$ and $\tau$
			are "compatible",
		\item \emph{associativity:} for all $\type{x}{\rho}, \type{y}{\sigma}, \type{z}{\tau} \in \?A$, if $\rho, \sigma, \tau$ are "compatible", then
		\[
			(\type{x}{\rho} \cdot \type{y}{\sigma}) \cdot \type{z}{\tau} 
			= \type{x}{\rho} \cdot (\type{y}{\sigma} \cdot \type{z}{\tau}).
		\]
		\item \emph{compatibility:} for all $\type{x}{\sigma}, \type{x'}{\sigma'}, \type{y}{\tau} \in \?A$, if $\type{x}{\sigma} \dep \type{x'}{\sigma'}$ and
		both $\sigma,\tau$ and $\sigma', \tau$ are "compatible", then
		$\type{x}{\sigma}\cdot \type{y}{\tau} \dep \type{x'}{\sigma'}\cdot \type{y}{\tau}$;\\
		dually if $\tau,\sigma$ and $\tau, \sigma'$ are "compatible", then 
		$\type{y}{\tau}\cdot \type{x}{\sigma} \dep \type{y}{\tau}\cdot \type{x'}{\sigma'}$.
	\end{itemize}
\end{definition}

In other words, a "positive synchronous algebra" is like a "synchronous algebra", potentially without units. Note that the restriction of a "positive synchronous algebra" $\?A$ to
its elements of "type" $\ll$, $\lb$ or $\bl$ yields three semigroups, called
the \AP""underlying semigroups"" of $\?A$. Moreover, any semigroup $S$ \AP""induces@@syncP""
a "positive synchronous algebra" \AP$\intro*\inducedalgSg{S}$, obtained by taking one copy of the semigroup for each "type",
and making all elements issued from the same element of the semigroup "dependent".
In fact, any semigroup morphism $\phi\colon (\SigmaPair)^+ \to S$ \reintro(syncP){induces}
a "morphism of positive synchronous algebras" \AP$\intro*\inducedmorSg{\phi}\colon \SyncP\Sigma \to \inducedalgSg{S}$.
\AP""Morphisms of positive synchronous algebras"" are defined as "maps of typed sets" which preserve
the "type".
Note that by definition, in any "synchronous algebra", there exists elements which
are "dependent" but not equal, because of the units. This is not true for "positive algebras@@sync".

\subparagraph*{Free algebras.} Let \AP$\intro*\SyncP\Sigma$ be the "dependent set" defined by:
\begin{itemize}
	\item $\SyncP{\Sigma}_{\ll} \defeq (\Sigma\times \Sigma)^+$,
	\item $\SyncP{\Sigma}_{\ll\to\lb} \defeq (\Sigma\times \Sigma)^+(\Sigma\times \pad)^+$,
	\item $\SyncP{\Sigma}_{\lb} \defeq (\Sigma\times \pad)^+$,
	\item $\SyncP{\Sigma}_{\ll\to\bl} \defeq (\Sigma\times \Sigma)^+(\pad\times \Sigma)^+$,
	\item $\SyncP{\Sigma}_{\bl} \defeq (\pad\times \Sigma)^+$,
	\item $\dep$ is the equality relation.
\end{itemize}
Together with natural concatenation, this defines a "positive synchronous algebra", which is moreover free, in the sense that
"positive synchronous algebra morphisms" from $\SyncP{\Sigma} \to \?A$ are in bijection
with "maps of typed sets" $\SigmaPair \to \?A$.
Every relation
$\+R \subseteq \Sigma^* \times \Sigma^* \smallsetminus \{(\varepsilon, \varepsilon)\}$
induces a unique "closed subset", denoted by \AP$\intro*\projP{\+R}$, of $\SyncP\Sigma$.

\subsection{Properties of Positive Algebras}
\label{sec:properties-positive-algebras}

The whole setting developed in \Cref{sec:synchronous-algebras} can be easily adapted to 
deal with "positive algebras@@sync".

\begin{proposition}[Syntactic morphism theorem]
	\label{lem:syntactic-morphism-theorem-positive}
	For each relation $\+R \subseteq \Sigma^*\times\Sigma^* \smallsetminus \{(\varepsilon, \varepsilon)\}$, there exists a surjective "synchronous positive morphism"
	\[\AP\intro*\SyntSAMP{\+R}\colon \Sync{\Sigma} \surj \intro*\SyntSAP{\+R}\]
	which "recognizes@@sync" $\+R$ and is such that for any other
	surjective "synchronous positive morphism"
	$\phi\colon \Sync{\Sigma} \surj \?B$
	"recognizing@@sync" $\+R$, there exists a
	"synchronous positive morphism" $\psi \colon \?B \surj \SyntSA{\+R}$
	such that the diagram
	\begin{center}
		\begin{tikzcd}
			\Sync\Sigma
				\ar[r, "\SyntSAMP{\+R}", twoheadrightarrow]
				\ar[dr, "\phi" swap, twoheadrightarrow]
			& \SyntSAP{\+R} \\
			& \?B, \ar[u, "\psi" swap, twoheadrightarrow]
		\end{tikzcd}
	\end{center}
	commutes.
	Objects $\SyntSAMP{\+R}$ and $\SyntSAP{\+R}$ are called the \AP""syntactic positive synchronous algebra morphism""
	and \AP""syntactic positive synchronous algebra"" of $\+R$, respectively.
	Moreover, these objects are unique up to "isomorphisms" of the "algebra@@syncP".
\end{proposition}

"Congruences@@sync", "quotient structures@@sync" and
"syntactic congruences@@sync" are defined in the
same way as for "synchronous algebras", modulo units, see \Cref{sec:syntactic-morphism}.

\begin{proposition}
	For any "positive synchronous algebra morphism" $\phi\colon \SyncP\Sigma \to \?A$
	"recognizing@@sync" a "relation" $\+R \subseteq (\Sigma^* \times \Sigma^*) \smallsetminus \{(\varepsilon, \varepsilon)\}$, say $\projP{\+R} = \phi^{-1}[\Acc]$, then 
	\begin{center}
		\begin{tabular}{rccc}
			$\quotient{\phi}{\congr{\Acc}}\colon$
			& $\SyncP\Sigma$
			& $\surj$
			& $\quotient{\?A}{\congr{\Acc}}$\\
			& $u$
			& $\mapsto$
			& $\equivclass{\phi(u)}{\congr{\Acc}}$
		\end{tabular}		
	\end{center}
	is the "syntactic morphism@@syncP" of $\+R$.
\end{proposition}

\begin{corollary}
	\label{coro:syntactic-congruence-is-syntactic-dependency-positive}
	In the "syntactic positive synchronous algebra" $\SyntSAP{\+R}$, the "syntactic
	congruence" $\congr{\Acc}$ and the "dependency relation" $\dep$
	coincide. 
\end{corollary}

\subparagraph*{Consolidation of the "syntactic positive synchronous algebra".}
Lastly, note that one key difference between the two settings is that any word
$u \in (\SigmaPair)^+$ can be unambiguously identified as a unique word of
$(\Sigma^* \times \Sigma^*) \smallsetminus \{(\varepsilon, \varepsilon)\}$.
This leads to some nice relationship between the "consolidation"
of the "syntactic positive synchronous algebra" of $\+R$
and its syntactic semigroup (when seen as a language over $\SigmaPair$). In short,
the "consolidation"\footnote{Defined analogously to the "consolidation" of a "synchronous algebra", except that the units are not merged---it would be hard to merge what does not exist.} of the "syntactic positive synchronous algebra" of $\+R$ is the smallest semigroup recognizing $\+R$, which can be $\types$-typed.
The "consolidation" of a "positive algebra@@sync" is defined similarly to the "consolidation" of
an "algebra@@sync". Consider the "consolidation" $\consolSyntSAP{\+R}$ of
the "syntactic positive algebra@@sync".

The unique "morphism@@sync" $\SyntSAP{\+R} \to \?1$ induces a 
semigroup morphism \AP$\intro*\projtype\colon \consolSyntSAP{\+R} \to \consol{\?1}$ where $\?1$
is the trivial "positive synchronous algebra" which has one element of each "type" on which
$\dep$ is the full relation. Elements of $\consol{\?1}$ can be thought as "types" or zero,
and $\projtype$ assigns to every element of $\SyntSAP{\+R}$ to its "type", and
maps $0 \in \consolSyntSAP{\+R}$ to $0 \in \consol{\?1}$.
Similarly, there is a map assigning to each word of $(\SigmaPair)^+$
its "type" or $0$. This semigroup morphism is denoted by
\AP$\intro*\typemap\colon (\SigmaPair)^+ \to \consol{\?1}$.
Note in fact that $\consol{\?1}$ is the syntactic semigroup of $\WellFormed$.

On the other hand $\SyntSAMP{\+R}\colon \SyncP\Sigma \surj \SyntSAP{\+R}$
induces a semigroup morphism $\consolSyntSAMP{\+R}\colon \consol{(\SyncP\Sigma)} \surj \consolSyntSAP{\+R}$. But then note that there is a canonical surjective morphism
$\sigma\colon (\SigmaPair)^+ \to \consol{(\SyncP\Sigma)}$: it sends
a "well-formed word" to its corresponding element, and a "non-well-formed word" to $0$.
Then, by construction
$\consolSyntSAMP{\+R} \circ \sigma\colon (\SigmaPair)^+ \surj \consolSyntSAP{\+R}$
recognizes $\+R$, seen as a subset of $(\SigmaPair)^+$: we denote this "morphism@@syncP"
by \AP$\intro*\sgpSyntSAMP{\+R}$.
So, letting
\[
	\zeta_{\+R}\colon
	(\SigmaPair)^+ \surj S_{\+R}
\]
denote the syntactic semigroup morphism of $\+R$,
by definition, there exists a surjective semigroup morphism
\AP$\intro*\projval\colon \consolSyntSAP{\+R} \to S_\+R$, such that
$\projval \circ \sgpSyntSAMP{\+R} = \zeta_{\+R}$.

\begin{proposition}
	\label{prop:consolidation}
	The following diagram commutes:
	\begin{center}
	\begin{tikzcd}[row sep=large]
		&
		(\SigmaPair)^+
			\dar["\vphantom{\hat{\eta}}\sgpSyntSAMP{\+R}" description, twoheadrightarrow]
			\ar[dl, "\typemap" swap, twoheadrightarrow]
			\ar[dr, "\zeta_{\+R}", twoheadrightarrow]&
		\\
		\consol{\?1} &
		\consolSyntSAP{\+R}
			\lar["\projtype", twoheadrightarrow]
			\rar["\projval" swap, twoheadrightarrow] &
		S_{\+R}.
	\end{tikzcd}
	\end{center}
\end{proposition}

In other words, every element of $\consolSyntSAP{\+R}$ 
can be assigned both a type-ish (namely an element of $\consol{\?1}$) and
a value (in the syntactic semigroup $S_{\+R}$ of $\+R$) consistently
with the types and values of $(\SigmaPair)^+$. In fact, we can show that
it is the \emph{canonical} object satisfying this property,
see \Cref{apdx:canonicity-consolidation}.

\subsection{Pseudovarieties \& Profinite Dependencies}

While many of the elementary properties of
"synchronous algebras"---and monoids and semigroups---remain true on "positive synchronous algebras", "eg" the existence of syntactic algebras, or the "Eilenberg correspondence@@sync" between
varieties of relations and varieties of algebras, the "Lifting Theorem" fails.
For instance, there are "relations" whose "underlying semigroups"
of their "syntactic positive synchronous algebra" are all groups,
but these "relations" are not "group relations"!

\begin{example}[Group relations: \Cref{ex:charac-group-relation-monoids}, cont'd.]
	\label{ex:counter-ex-group-relations-semigroups}
	Consider the relation $\+R \defeq \{(u, v) \mid u > v \text{ and } |u| \equiv |v| \bmod{p}\}$.
	Then the "underlying semigroups" of the "syntactic positive synchronous algebra" of $\+R$
	of "type" $\ll$, $\lb$, $\bl$ are groups---namely $\Z/1\?Z$, $\Z/p\?Z$ and $\Z/1\?Z$, respectively. Yet, $\+R$ is not a "group relation".
\end{example}

So, in order to still manage to characterize "$\+V$-relations" via their 
"syntactic positive synchronous algebras", we will introduce
"profinite dependencies"---which are the equivalent of ``profinite equalities''
adapted to our setting---and show a Reiterman-style result---namely that
"pseudovarieties of positive synchronous algebras" are exactly the class
of "positive synchronous algebras" characterized by "profinite dependencies".
Our results rely on an adaptation of the theory of profinite words to our settings:
we follow \cite[\S X—XIII]{pin_mathematical_2022}, and most proof can be caried
to our setting with ease.

\AP""Pseudovarieties of positive synchronous algebras"" are defined as classes of "locally 
generated" finite "positive synchronous algebras" closed under Cartesian product and 
"division@@sync". A ""$+$-pseudovariety of synchronous relations"" is a class
$\+V\colon \Sigma \mapsto \+V_{\Sigma}$ "st" for any finite alphabet $\Sigma$,
$\+V_{\Sigma}$ is a set of "synchronous relations"
$\+R \subseteq (\Sigma^*\times\Sigma^*) \smallsetminus \{(\varepsilon, \varepsilon)\}$
closed under "Boolean combinations", "syntactic derivatives" and "inverse morphisms"
of free "positive synchronous algebras".

\begin{remark}
	Note that the last condition is the main difference with
	"$*$-pseudovariety of synchronous relations", since "morphisms of positive synchronous algebras"
	\[
		\phi\colon \SyncP\Gamma \to \SyncP\Sigma
	\]
	have to be non-erasing, "ie" $\phi(u) \neq \varepsilon$, contrary to
	"morphisms of synchronous algebras" from $\Sync\Gamma \to \Sync\Sigma$. This implies
	that the closure properties imposed to be a "$+$-pseudovariety@@sync" are much weaker
	than those imposed to be "$\ast$-pseudovariety@@sync".
\end{remark}

\begin{lemma}
	\label{lemma:characterization-pseudovarieties-syncrel-positive}
	A class $\+V\colon \Sigma \mapsto \+V_\Sigma$ is a "$+$-pseudovariety of synchronous relations" if, and only if, it is closed under "Boolean combinations", "residuals" and
	"inverse morphisms" of free "positive synchronous algebras".
\end{lemma}

\begin{lemma}[An Eilenberg theorem for positive synchronous relations]
	\label{lem:eilenberg-sy-positive}
	The correspondences $\B{V} \corrAR \+V$ and $\+V \corrRA \B{V}$ define
	mutually inverse bijective correspondences between "pseudovarieties of
	positive synchronous algebras" and "$+$-pseudovarieties of synchronous relations".
\end{lemma}

We then adapt a classical result from algebraic language theory, known
as Reiterman's theorem \cite[Theorem 3.1, p.~4]{reiterman_birkhoff_1982} \cite[Theorem XI.3.13, p.~195]{pin_mathematical_2022}, that shows that pseudovarieties of semigroups are exactly the
classes of finite semigroups defined by ``profinite equalities''---"eg" commutative semigroups
are exactly the semigroups satisfying $xy = yx$, and aperiodic semigroups 
are those satisfying $x^{\idem+1} = x^{\idem}$ where $-^{\idem}$ denotes the "idempotent power".

\subparagraph*{Profinite words.}
Given a "typed set" $X$ with only elements of type
$\ll,\lb,\bl$,\footnote{This assumption is there because we are only interested in "locally generated algebras".} consider the space\footnote{We only gave a definition
of this when $X$ had the form $\SigmaPair$ but given a more general definition is quite easy,
see \Cref{apdx:monads}.} $\SyncP X$ of all words over $X$ equipped with the ultrametric
\AP\phantomintro{\dist}\phantomintro{\rist}
\begin{align*}
	\reintro*\dist(u,v) & \defeq 2^{-\rist(u,v)} \text{ where } \\
	\reintro*\rist(u,v) & \defeq 
	\min{\bigl\{n\in \N \mid}
	\text{ $\phi(u) \neq \phi(v)$ for some "positive@positive algebra@sync"} \\[-.2em]
	& \hphantom{\defeq \min{\bigl\{n\in \N \mid}}
		\text{ "synchronous algebra morphism@positive algebra@sync" $\phi$} \\[-.35em]
	& \hphantom{\defeq \min{\bigl\{n\in \N \mid}}
		\text{ whose codomain has at most $n$ elements}\bigr\}.
\end{align*}

\AP We then consider ""Cauchy sequences"" of words over $X$, 
namely sequences $(u_n)_{n\in\N} \in (\SyncP X)^{\smash{\N}}$ such that
for every $\varepsilon > 0$, there exists $n_\varepsilon > 0$ such that
for all $p,q \geq n_{\varepsilon}$, we have $\dist(u_p, u_q) \leq \varepsilon$.
Say that two "Cauchy sequences" $(u_n)_{n\in\N}$ and $(v_n)_{n\in\N}$ are equivalent when 
for every $\varepsilon > 0$, then eventually always $\dist(u_n,v_n) \leq \varepsilon$.

Notice that if two words $u$ and $v$ have different "type", then
$\rist(u,v) = |\types|$, "ie" it is equal to the size of the trivial "positive algebra@@sync".
In particular, in a "Cauchy sequence", all words must eventually all have the same "type",
and this is how we define the "type" of a "Cauchy sequence".

\begin{definition}
	""Profinite words"" over $X$ are defined as the space of Cauchy sequences,
	up to equivalence, together with the metric induced by $\dist$.
	They form a compact topological space, denoted by \AP$\intro*\profSy{\SyncP X}$. Moreover,
	when equipped with piecewise concatenation, $\profSy{\SyncP X}$ is a "positive synchronous 
	algebra" where the "dependency relation" coincides with equality.
\end{definition}

Note that, by definition, any "morphism of positive synchronous algebras"
$\phi\colon \SyncP X \to \?A$, where $\?A$ is finite,
can be extended to $\reintro*\profSy{\phi}\colon \profSy{\SyncP X} \to \?A$ by letting $\profSy{\phi}(\equivclass{(u_n)_{n\in\N}}{})$ be the stationary value of $(\phi(u_n))_{n\in\N}$.
For instance, if $x$ has "type" $\tau \in \{\ll, \lb, \bl\}$, then $((\type{x}{\tau})^{n!})_{n\in \N}$
is a "Cauchy sequence", whose equivalence class is denoted by \AP$\type[\intro*\idem]{x}{\tau}$, and $\profSy{\phi}(\type[\idem]{x}{\tau})$ is the unique \AP""idempotent power"" of
$\phi(\type{x}{\tau})$ in the "underlying semigroup" of "type" $\tau$.\footnote{In other words, it is the 
unique element $e$ of the form $\type[n]{x}{\tau}$ with $n\in \Np$ "st" $e = e\cdot e$. See \cite[\S II.6, p.~32]{pin_mathematical_2022} for more details.}
On the other hand, note that it does not make sense to speak about the "idempotent power"
of an element of type $\ll\to\lb$ or $\ll \to \bl$. 

\begin{definition}
	Let $X$ be a finite "typed set". A \AP""profinite dependency"" over variables $X$,
	consists of a pair $(\type{u}{\sigma}, \type{v}{\tau}) \in \profSy{\SyncP X}$ denoted by \AP$u \intro*\profdep v$.
	A "positive synchronous algebra" $\?A$ \AP""satisfies@@profdep"" this "profinite dependency"
	when for all "morphisms@@syncP"\footnote{Which are in bijection
	with "maps of typed sets" from $X$ to $\?A$, and so it can be thought of a valuation
	of variables from $X$ with values in $\?A$.} $\phi\colon \SyncP X \to \?A$, $\profSy{\phi}(\type{u}{\sigma}) \dep^{\?A} \profSy{\phi}(\type{v}{\tau})$.
\end{definition}

More generally, if $\+E$ is a (potentially infinite) set of "profinite dependencies"
and $\B{V}$ is a class of "positive synchronous algebras", we say that $\B{V}$
\reintro(profdep){satisfies} $\+E$ when all $\?A \in \B{V}$ "satisfy@@profdep" 
all $(\type{u}{\sigma} \profdep \type{v}{\tau}) \in \+E$.
We say that $\B{V}$ is ""defined@@profdep"" by $\+E$ when $\B{V}$
is exactly the set \AP$\intro*\semprofdep{\+E}$ of all "positive algebras@@sync" that
"satisfy@@profdep" $\+E$.

\AP\phantomintro(sync){Reiterman-style characterization of pseudovarieties}\vspace{-1em}
\begin{restatable}[\reintro(sync){A Reiterman theorem for positive synchronous algebras}]{theorem}{lemmareiterman}
	\label{thm:reiterman-sy}
	A class of "locally generated" finite "positive synchronous algebras" is
	a "pseudovariety@@syncP" if, and only if, it is "defined@@profdep" by a
	set of "profinite dependencies".\footnote{Note however that this set
	can be infinite.}
	Moreover, "wlog", all variables have type $\ll$, $\lb$ or $\bl$.
\end{restatable}

The proof can be adapted from \cite[\S XI.3.3, pp.~194--196]{pin_mathematical_2022},
see \Cref{apdx-proof:profinite-pseudovar}.
Note also that a similar statement holds for (non-positive) "synchronous algebras".

% \subsection{Some Natural Pseudovarieties}
% \label{sec:ex-pseudovarieties}

% \begin{proposition}
% 	\label{prop:recognizable-is-pseudovariety}
% 	The class of all "recognizable relations" is a "$*$-pseudovariety of synchronous relations".
% \end{proposition}

% \todo{proof}

% Say that a "relation" $\+R$ is \AP""almost length-preserving"", "aka" has \reintro{bounded length discrepancy}, if there exists $k \in \N$ such that for all $(u, v) \in \+R$,
% then $||u|-|v|| \leq k$.

% \begin{proposition}
% 	\label{prop:alp-is-pseudovariety}
% 	The Boolean closure of "almost length-preserving relations" is not
% 	a "$*$-pseudovariety of synchronous relations", but is a "$+$-pseudovariety@@sync".
% 	% Moreover, the "corresponding@@EilenbergSy" "pseudovariety of positive synchronous algebras"
% 	% is characterized by the "profinite dependencies"
% 	% \begin{align}
% 	% 	& \type[\idem]{x}{\lb} \type{y}{\lb} \profeq \type[\idem]{x}{\lb}, &
% 	% 	\type{y}{\sigma} \type[\idem]{x}{\lb} \profdep \type[\idem]{x}{\lb}, \label{eq:alp-lb}\\
% 	% 	& \type[\idem]{x}{\bl} \type{y}{\bl} \profeq \type[\idem]{x}{\bl}, &
% 	% 	\type{y}{\sigma} \type[\idem]{x}{\bl} \profdep \type[\idem]{x}{\bl}, \label{eq:alp-bl}\\
% 	% 	& \type[\idem]{x}{\lb} \profdep \type[\idem]{x}{\bl} \label{eq:alp-zero}.
% 	% \end{align}
% \end{proposition} 

% \todo{proof}
